FRAME: Fast and Realistic Attacker Modeling and Evaluation for Temporal Logical Correlation in Static Noise

We propose a method called Fast and Realistic Attacker Modeling and Evaluation (FRAME) that can reduce pessimism in static noise analysis by exploiting temporal logical correlation of attackers and using novel techniques termed envelopes and $\sigma$ functions. Unlike conventional pruning-based approaches, FRAME efficiently considers all relevant attackers, thereby producing more realistic results. FRAME was tested with complex industrial design and successfully reduced the pessimism of conventional techniques by 30.4% on average, with little computational overhead.

==> reference.tex <==
\begin{thebibliography}{10}

\bibitem{arun01}
R.~Arunachalam, R.~D. Blanton, and L.~T. Pileggi.
\newblock False coupling interactions in static timing analysis.
\newblock In {\em Proc. {IEEE/ACM} DAC}, pages 726-- 731, June 2001.

\bibitem{becer05}
M.~Becer, V.~Zolotov, R.~Panda, A.~Grinshpon, I.~Algol, R.~Levy, and C.~Oh.
\newblock Pessimism reduction in crosstalk noise aware {STA}.
\newblock In {\em Proc. {IEEE/ACM} ICCAD}, pages 954--961, November 2005.

\bibitem{chai03}
D.~Chai, A.~Kondratyev, Y.~Ran, K.~Tseng, Y.~Watanabe, and M.~Marek-Sadowska.
\newblock Temporofunctional crosstalk noise analysis.
\newblock In {\em Proc. {IEEE/ACM} DAC}, pages 860--863, June 2003.

\bibitem{chen01}
L.~H. Chen and M.~Marek-Sadowska.
\newblock Aggressor alignment for worst-case crosstalk noise.
\newblock {\em {IEEE} TCAD}, 20(5):612--621, May 2001.

\bibitem{chen99}
P.~Chen and K.~Keutzer.
\newblock Towards true crosstalk noise analysis.
\newblock In {\em Proc. {IEEE/ACM} ICCAD}, pages 132--137, November 1999.

\bibitem{das08}
D.~Das, K.~Killpack, C.~Kashyap, A.~Jas, and H.~Zhou.
\newblock Pessimism reduction in coupling-aware static timing analysis using
  timing and logic filtering.
\newblock In {\em Proc. ASPDAC}, pages 486--491, March 2008.


\bibitem{glebov02}
A.~Glebov, S.~Gavrilov, D.~Blaauw, V.~Zolotov, R.~Panda, and C.~Oh.
\newblock False-noise analysis usng resolution method.
\newblock In {\em Proc. ISQED}, pages 437--442, March 2002.

\newpage


\bibitem{glebov04}
A.~Glebov, S.~Gavrilov, R.~Soloviev, V.~V~Zolotov, M.~R. Becer, C.~Oh, and
  R.~Panda.
\newblock Delay noise pessimism reduction by logic correlations.
\newblock In {\em Proc. {IEEE/ACM} ICCAD}, pages 160--167, November 2004.

\bibitem{glebov02acm}
A.~Glebov, S.~Gavrilovand, D.~Blaauw, and V.~Zolotov.
\newblock False-noise analysis using logic implications.
\newblock {\em ACM TODAES}, 7(3):474--498, July 2002.

\bibitem{lee04}
H.~Lee and J.~Kim.
\newblock False aggressors pruning using path sensitization and logic
  implications.
\newblock In {\em Proc. ASPDAC}, pages 278--281, August 2004.

\bibitem{palla08}
M.~Palla, J.~Bargfrede, K.~Koch, W.~Anheier, and R.~Drechsler.
\newblock Adaptive branch and bound using {SAT} to estimate false crosstalk.
\newblock In {\em Proc. ISQED}, pages 508--513, March 2008.

\bibitem{palla06}
M.~Palla, K.~Koch, J.~Bargfrede, M.~Glesner, and W.~Anheier.
\newblock Reduction of crosstalk pessimism using tendency graph approach.
\newblock In {\em Proc. ICCD}, pages 50--55, October 2006.

\bibitem{ran05}
Y.~Ran, A.~Kondratyev, K.~H. Tseng, Y.~Watanabe, and M.~{Marek-Sadowska}.
\newblock Eliminating false positives in crosstalk noise analysis.
\newblock {\em {IEEE} TCAD}, 24(9):1406--1419, September 2005.

\bibitem{rice95}
J.~A. Rice.
\newblock {\em Mathematical Statistics and Data Analysis}.
\newblock Duxbury Press, Belmont, California, 1995.

\bibitem{tehrani00}
P.~Tehrani, S.~W. Chyou, and U.~Ekambaram.
\newblock Deep sub-micron static timing analysis in presence of crosstalk.
\newblock In {\em Proc. ISQED}, pages 505--512, March 2000.

\bibitem{tseng05}
K.~Tseng and M.~Horowitz.
\newblock False coupling exploration in timing analysis.
\newblock {\em {IEEE} TCAD}, 24(11):1795--1805, November 2005.

\bibitem{xiao00b}
T.~Xiao, C.-W. Chang, and M.~Marek-Sadowska.
\newblock Efficient static timing analysis in presence of crosstalk.
\newblock In {\em Proc. {ASIC/SOC}}, pages 335--339, September 2000.

\bibitem{xiao01}
T.~Xiao and M.~Marek-Sadowska.
\newblock Functional correlation analysis in crosstalk induced critical paths
  identification.
\newblock In {\em Proc. {IEEE/ACM} DAC}, pages 653--656, June 2001.

\bibitem{xiao00}
T.~Xiao, M.~Marek-Sadowska, and M.~Worst.
\newblock Delay estimation in crosstalk aware static timing analysis.
\newblock In {\em Proc. {ICCD}}, pages 115--120, September 2000.

\bibitem{yang03}
J.-S. Yang, J.-Y. Kim, J.-H. Choi, M.-H. Yoo, and J.-T. Kong.
\newblock Elimination of false aggressors using the functional relationship for
  full-chip crosstalk analysis.
\newblock In {\em Proc. ISQED}, pages 344--347, March 2003.

\end{thebibliography}

